Liquid Cloud Storage

A liquid system provides durable object storage based on spreading redundantly generated data across a network of hundreds to thousands of potentially unreliable storage nodes. A liquid system uses a combination of a large code, lazy repair, and a flow storage organization. We show that a liquid system can be operated to enable flexible and essentially optimal combinations of storage durability, storage overhead, repair bandwidth usage, and access performance.

==> sect_related_work.tex <==
\section{Related work}
\label{related sec}

A substantial number of research papers are devoted to the topic of distributed cloud storage. 
A rather comprehensive and well organized repository can be found at \cite{DimakisR}.

\subsection{Erasure codes}

Many erasure codes have been developed over the years, including those described in  \cite{CCauchy95}, \cite{CAlon96}, \cite{CLuby97}, \cite{CRizzo97}, \cite{CLubyA98}, \cite{CLuby01}, \cite{CLubyA02}, \cite{CLuby02}, \cite{CMaymounkov02}, \cite{CRaptor06}, \cite{CRaptorQ11}, \cite{patD}, \cite{patC},  \cite{patB}, \cite{patE}, \cite{patF}, \cite{patG}, \cite{patH}, \cite{patK}, \cite{patM}, \cite{patP}, \cite{patN}, \cite{patL}, \cite{patT}, \cite{patU}.  Erasure codes have found a number of applications other than storage systems, some of which are described in \cite{APET96}, \cite{ADF98}, \cite{AMirror99}, \cite{AFLID00}, \cite{AWEBRC02}, \cite{ADF02}, \cite{AFLID02}, \cite{ABROAD06}, \cite{APOWER07}, \cite{ABROAD07}, \cite{AHANDBOOK08}, \cite{ASMPTE08}, \cite{AIPTV08}, \cite{ABESTPRAC12}.  Erasure codes have been adopted into a number of industrial standards, including \cite{RFC3453}, \cite{RFC3738}, \cite{MBMS}, \cite{DVBIPDC}, \cite{RFC5052}, \cite{DVBIPTV}, \cite{RFC5053}, \cite{DVBCDS}, \cite{OMA}, \cite{RFC5510}, \cite{RFC5651}, \cite{RFC5575}, \cite{RFC6330}, \cite{RFC6681}, \cite{RFC6726}.

\subsection{Locally recoverable codes}

{\em Local reconstruction codes} (LRC) have been introduced in \cite{Gopalan12}, \cite{Dimakis13}.  For example, compared to $(18,12,2,2)$ LRC codes in terms of repair bandwidth.

\subsection{Regenerating codes}

{\em Regenerating codes} have been introduced in \cite{Dimakis07}, \cite{Dimakis10}.  These include {\em Minimum Storage Regenerating codes} (MSR codes) and {\em Minimum Bandwidth Regenerating codes} (MBR codes).

\subsection{Lazy repair}

Lazy repair comparison from \cite{Quantitative02}, i.e., has idea of repair epoch and lazy repair can be done, but very little details (only theoretical), and bound on \mttl\ depends on number of objects stored.  Also, lazy repair in different sense, i.e., deferring repair till at least a certain number of fragments have been lost, etc.

\subsection{Transient failures}

Many papers can be cited stating that 90\% of the failures are transient.  Also, mention issues with repairing due to transient failures is a big issue.

\subsection{Forward replication}

Proactive repair~\cite{Proactive06}

\subsection{\Placegroup s}

\subsection{Access}

\cite{Soljanin09} ? and others have results which show improved access when more than $k$ of $k$ fragments are requested.



